More Than Meets The Eye: Semi-supervised Learning Under Non-IID Data

A common heuristic in semi-supervised deep learning (SSDL) is to select unlabelled data based on a notion of semantic similarity to the labelled data. For example, labelled images of numbers should be paired with unlabelled images of numbers instead of, say, unlabelled images of cars. We refer to this practice as semantic data set matching. In this work, we demonstrate the limits of semantic data set matching. We show that it can sometimes even degrade the performance for a state of the art SSDL algorithm. We present and make available a comprehensive simulation sandbox, called non-IID-SSDL, for stress testing an SSDL algorithm under different degrees of distribution mismatch between the labelled and unlabelled data sets. In addition, we demonstrate that simple density based dissimilarity measures in the feature space of a generic classifier offer a promising and more reliable quantitative matching criterion to select unlabelled data before SSDL training.

==> tables/correlations.tex <==

\begin{table}[t]
%\begin{table}[t]
\caption{Correlation results for the dissimilarity measures between $S_l$ and $S_u$ with  \gls{OOD} contamination and  \gls{SSDL} accuracy.}
\label{tab:correlations}
\begin{center}


\begin{tabular}{cccccc}
\toprule
\textbf{$\mathbf{S_l}$}       & \textbf{$\mathbf{n_l}$} & \textbf{$\mathbf{d_{\ell_1}}$} & \textbf{$\mathbf{d_{\ell_2}}$} & \textbf{$\mathbf{d_{JS}}$} & \textbf{$\mathbf{d_{C}}$} \\ \hline
\multirow{3}{*}{MNIST}        & 60                      & -0.876                         & -0.898                         & -0.969                     & -0.944                    \\
                              & 100                     & -0.805                         & -0.83                          & -0.786                     & -0.948                    \\
                              & 150                     & -0.794                         & -0.822                         & -0.81                      & -0.944                    \\ \hline
\multirow{3}{*}{CIFAR-10}     & 60                      & -0.823                         & -0.853                         & -0.944                     & -0.921                    \\
                              & 100                     & -0.826                         & -0.878                         & -0.966                     & -0.947                    \\
                              & 150                     & -0.808                         & -0.838                         & -0.952                     & -0.927                    \\ \hline
\multirow{3}{*}{FashionMNIST} & 60                      & -0.2                           & -0.268                         & -0.735                     & -0.789                    \\
                              & 100                     & -0.264                         & -0.326                         & -0.781                     & -0.824                    \\
                              & 150                     & -0.286                         & -0.347                         & -0.785                     & -0.827                    \\  
\bottomrule
\end{tabular}

\end{center}
%\end{table}
\end{table}

==> tables/half-half-results-v2.tex <==
\begin{table}
\caption{TBD}
\label{tab:half-half-results}
\begin{center}
\begin{small}

%l@{\qquad}c@{\;\;}c@{\qquad}c@{\;\;}c
\begin{tabular}{lccccccccc}
\toprule
 & \multicolumn{3}{c}{\textbf{MNIST}} 
 & \multicolumn{3}{c}{\textbf{CIFAR-10}}
 & \multicolumn{3}{c}{...} \\
 
   $N$ labelled 
 & 0 
 & 50 
 & 100
 & 0 
 & 50 
 & 100
 & 0 
 & 50 
 & 100 \\
 
 \midrule

   60 
 & $99\pm0.01$
 & $99\pm0.01$ 
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$ \\
 
   100
 & $99\pm0.01$
 & $99\pm0.01$ 
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$ \\
 
  150
 & $99\pm0.01$
 & $99\pm0.01$ 
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$
 & $99\pm0.01$ \\
 
 \midrule
 Baseline
 & \multicolumn{3}{c}{$99\pm0.01$} 
 & \multicolumn{3}{c}{$99\pm0.01$}
 & \multicolumn{3}{c}{$99\pm0.01$}\\
 

 \bottomrule
\end{tabular}

\end{small}
\end{center}
\end{table}

==> tables/half-half-results.tex <==
\begin{table}
\caption{Results for OOD Type "Half-Half". Half-half means that the model only learns to predict on half of classes present in the data set. The data from the other half of classes is used as OOD data. OOD \% denotes the percentage of OOD data in the unlabeled data used for semi-supervised training. $N$ labelled denotes the number of labeled data points from the IOD data that were used during semi-supervised training. BL denotes a baseline, fully-supervised model that was trained on all labelled IOD data.}
\label{tab:half-half-results}
\begin{center}
\begin{small}

%l@{\qquad}c@{\;\;}c@{\qquad}c@{\;\;}c
\begin{tabular}{cc|ccc|c}
\toprule
 & & \multicolumn{3}{c|}{$N$ Labelled} & BL \\

Data Set & OOD \% & 60 & 100 & 150 & \\
\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{MNIST}}} & 60 & $00\pm0.00$ & $00\pm0.00$ & $00\pm0.00$ & \multirow{3}{*}{\textbf{$00\pm0.00$}} \\
 & 100 & $00\pm0.00$ & $00\pm0.00$ & $00\pm0.00$ & \\
 & 150 & $00\pm0.00$ & $00\pm0.00$ & $00\pm0.00$ & \\
\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{CIFAR}}} & 60 & $00\pm0.00$ & $00\pm0.00$ & $00\pm0.00$ & \multirow{3}{*}{\textbf{$00\pm0.00$}} \\
 & 100 & $00\pm0.00$ & $00\pm0.00$ & $00\pm0.00$ & \\
 & 150 & $00\pm0.00$ & $00\pm0.00$ & $00\pm0.00$ & \\
\midrule
\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{...}}} & 60 & $00\pm0.00$ & $00\pm0.00$ & $00\pm0.00$ & \multirow{3}{*}{\textbf{$00\pm0.00$}} \\
 & 100 & $00\pm0.00$ & $00\pm0.00$ & $00\pm0.00$ & \\
 & 150 & $00\pm0.00$ & $00\pm0.00$ & $00\pm0.00$ & \\

 \bottomrule
\end{tabular}

\end{small}
\end{center}
\end{table}

==> tables/results-backup.tex <==
\begin{table*}[]
%\caption{\textbf{Results OOD Experiments.} IOD Data is the base data set that is considered IOD. OOD Type is the OOD configuration which can be \textit{half-half} (the model only learns to predict on half of the classes present in the data set while the data from the OH of classes is used as OOD data) or \textit{different} (data sets from a different data set than the IOD data are used as OOD data). OOD Data signifies the data set that was used as OOD data. OOD \% is the percentage of OOD data in the unlabeled data. $N$ Labelled is the number of labelled data points from IOD Data that were used during semi-supervised training. BL is the performance of a fully supervised baseline model trained on the entire data set of labelled IOD Data.}
\caption{Results for the class distribution mismatch experiment. Each result entry in the table represents the mean and variance of accuracy across ten random experimental runs per entry. For a detailed description of symbols and the experiment see \Cref{sec:testbed}.}
\label{tab:half-half-results}
%\begin{center}
%\begin{tiny}

\centering
%l@{\qquad}c@{\;\;}c@{\qquad}c@{\;\;}c
\begin{tabular}{ccccccc}
\toprule
\multirow{2}{*}{$\mathbf{S_{IOD}}$} & \multirow{2}{*}{$\mathbf{T_{OOD}}$} & \multirow{2}{*}{$\mathbf{S_{uOOD}}$} & \multirow{2}{*}{$\mathbf{\%_{uOOD}}$} & \multicolumn{3}{c}{$\mathbf{n_l}$}\\

&  & &  & 60 & 100 & 150\\

\midrule

\multirow{12}{*}{\rotatebox[origin=c]{90}{\textbf{MNIST}}} 
& \multicolumn{3}{c}{Fully supervised baseline} & $0.457\pm0.108$ & $0.559\pm 0.125 $ & $0.645 \pm0.101$ \\

 & \multicolumn{3}{c}{SSDL baseline (no OOD data)} & $\mathbf{0.704 \pm 0.096}$ & $\mathbf{0.781\pm 0.065}$ & $\mathbf{0.831 \pm0.0626}$\\
 
 
 \cline{2-7}
 
 & \multirow{2}{*}{HH} & \multirow{2}{*}{OH} & 50 & $0.679\pm0.108$ & $0.769\pm0.066$ & $0.802\pm0.054$\\
 & & & 100 & $0.642 \pm 0.111$ & $0.746 \pm0.094$ & $0.798 \pm0.07$\\
 
 
 \cline{2-7}
 & \multirow{2}{*}{Sim} & \multirow{2}{*}{SVHN} & 50 & $0.637 \pm0.098$ & $0.745 \pm0.081$ & $0.801 \pm0.0699$\\
 
 & & & 100 & $0.482 \pm0.113$ & $0.719 \pm0.058$ & $0.765 \pm0.072$\\
 
  \cline{2-7}
 
  & \multirow{6}{*}{Dif}& \multirow{2}{*}{TI} & 50 & $0.642 \pm0.094$ & $0.739 \pm 0.074$ & $0.809 \pm0.066$\\
  
  & & & 100 & $0.637 \pm0.097$ & $0.732\pm 0.074$ & $0.804 \pm0.071$\\
  
  
 
 \cline{3-7}
 
  & & \multirow{2}{*}{G} & 50 & $0.606 \pm0.0989$ & $0.713 \pm0.087$ & $0.786\pm 0.065$\\
  
  & & & 100 & $0.442 \pm0.099$ & $0.461 \pm0.073$ & $0.542\pm 0.062$\\
  
 
  
   \cline{3-7}
 
  & & \multirow{2}{*}{SAP} & 50 & $0.631 \pm0.102$ & $0.735 \pm0.082$ & $0.813 \pm0.057$\\
  
  & & & 100 & $0.48\pm0.0951$ & $0.524 \pm0.09$ & $0.563 \pm0.095$\\
 
\hline

\multirow{12}{*}{\rotatebox[origin=c]{90}{\textbf{CIFAR-10}}} & \multicolumn{3}{c}{Fully supervised baseline} & $0.380\pm0.024$ & $0.445\pm0.042$ & $0.449\pm0.022$\\

 &  \multicolumn{3}{c}{SSDL baseline (no OOD data)} & $\mathbf{0.453\pm0.046}$ & $0.474\pm0.019$ & $0.501\pm0.033$\\
 
 
 \cline{2-7}


& \multirow{2}{*}{HH} & \multirow{2}{*}{OH} & 50 & $0.444\pm0.040$ & $0.472\pm0.039$ & $0.525\pm0.050$\\ 
 & & & 100 & $0.443\pm0.023$ & $0.472\pm0.047$ & $0.499\pm0.054$ \\
 \cline{2-7}
 & \multirow{2}{*}{Sim} & \multirow{2}{*}{TI} & 50 & $0.435\pm0.054$ & $0.473\pm0.039$ & $\mathbf{0.543\pm0.040}$\\ 
 & & & 100 & $0.417\pm0.020$ & $\mathbf{0.480\pm0.039}$ & $0.498\pm0.042$ \\
 
 \cline{2-7}
 
  & \multirow{6}{*}{Dif} & \multirow{2}{*}{SVHN} & 50 & $0.419\pm0.027$ & $0.464\pm0.044$ & $0.469\pm0.056$\\ 
 & & & 100 & $0.385\pm0.034$ & $0.418\pm0.035$ & $0.440\pm0.046$ \\
 
 \cline{3-7}
 
  & & \multirow{2}{*}{G} & 50 & $0.409\pm0.047$ & $0.454\pm0.048$ & $0.491\pm0.032$\\ 
 & & & 100 & $0.297\pm0.029$ & $0.306\pm0.034$ & $0.302\pm0.038$ \\
 
 \cline{3-7}
 
  & & \multirow{2}{*}{SAP}& 50 & $0.438\pm0.029$ & $0.455\pm0.037$ & $0.485\pm0.034$\\ 
 & & & 100 & $0.236\pm0.031$ & $0.246\pm0.032$ & $0.232\pm0.022$ \\
  
  \hline

\multirow{12}{*}{\rotatebox[origin=c]{90}{\textbf{FashionMNIST}}} & \multicolumn{3}{c}{Fully supervised baseline} & $0.571\pm0.073$ & $0.704\pm0.066$ & $0.720\pm0.093$\\

 & \multicolumn{3}{c}{SSDL baseline (no OOD data)} & $\mathbf{0.715\pm0.049}$ & $\mathbf{0.760\pm0.044}$ & $0.756\pm0.069$\\
 \cline{2-7}

& \multirow{2}{*}{HH} & \multirow{2}{*}{OH} & 50 & $0.714\pm0.049$ & $0.721\pm0.104$ & $0.765\pm0.053$\\ 
 & & & 100 & $0.660\pm0.061$ & $0.711\pm0.090$ & $0.747\pm0.061$ \\
 \cline{2-7}
 & \multirow{2}{*}{Sim} & \multirow{2}{*}{FP} & 50 & $0.707\pm0.039$ & $0.724\pm0.030$ & $0.778\pm0.078$\\ 
 & & & 100 & $0.546\pm0.101$ & $0.542\pm0.099$ & $0.540\pm0.105$ \\
 
 \cline{2-7}
 
  & \multirow{6}{*}{Dif}& \multirow{2}{*}{TI} & 50 & $0.690\pm0.065$ & $0.745\pm0.093$ & $0.792\pm0.058$\\ 
 & & & 100 & $0.690\pm0.073$ & $0.728\pm0.066$ & $\mathbf{0.794\pm0.056}$ \\
  \cline{3-7}
  & & \multirow{2}{*}{G} & 50 & $0.644\pm0.061$ & $0.689\pm0.075$ & $0.755\pm0.055$\\ 
 & & & 100 & $0.352\pm0.025$ & $0.366\pm0.065$ & $0.361\pm0.057$ \\
  \cline{3-7}
  & & \multirow{2}{*}{SAP} & 50 & $0.671\pm0.072$ & $0.708\pm0.095$ & $0.729\pm0.088$\\ 
 & & & 100 & $0.276\pm0.069$ & $0.297\pm0.046$ & $0.283\pm0.059$\\
 \bottomrule
\end{tabular}
%\end{tiny}
%\end{center}
\end{table*}

==> tables/results-combined-June1-geneva1314.tex <==
\begin{table}
%\caption{\textbf{Results OOD Experiments.} IOD Data is the base data set that is considered IOD. OOD Type is the OOD configuration which can be \textit{half-half} (the model only learns to predict on half of the classes present in the data set while the data from the OH of classes is used as OOD data) or \textit{different} (data sets from a different data set than the IOD data are used as OOD data). OOD Data signifies the data set that was used as OOD data. OOD \% is the percentage of OOD data in the unlabeled data. $N$ Labelled is the number of labelled data points from IOD Data that were used during semi-supervised training. BL is the performance of a fully supervised baseline model trained on the entire data set of labelled IOD Data.}
\caption{$\mathbf{S_{IOD}}$: the dataset source used for the labelled data and the unlabelled IOD data, $\mathbf{T_{OOD}}$: type of unlabelled data used for the out of distribution setting (HH: half-half, Sim: human similar, Dif: human different), $\mathbf{S_{uOOD}}$: the dataset source used for the unlabelled OOD data (OH: other half, SVHN: Street View House Numbers, TI: Tiny ImageNet, G: Gaussian noise, SAP: Salt and pepper noise, FP: Fashion Product), $\mathbf{\%_{uOOD}}$: percentage of OOD data in the unlabelled data, $\mathbf{N_l}$: number of IOD labelled data points used in MixMatch training. Each result entry in the table represents the mean and variance of accuracy across ten random experimental runs per entry. For details about the runs please see the description in \Cref{sec:experiments}.}
\label{tab:half-half-results}
\begin{center}
\begin{small}


%l@{\qquad}c@{\;\;}c@{\qquad}c@{\;\;}c
\begin{tabular}{cccc|ccc}
\toprule
\multirow{2}{*}{$\mathbf{S_{IOD}}$} & \multirow{2}{*}{$\mathbf{T_{OOD}}$} & \multirow{2}{*}{$\mathbf{S_{uOOD}}$} & \multirow{2}{*}{$\mathbf{\%_{uOOD}}$} & \multicolumn{3}{c}{$\mathbf{N_l}$}\\

&  & &  & 60 & 100 & 150\\

\midrule

\multirow{12}{*}{\rotatebox[origin=c]{90}{\textbf{MNIST}}} 
& \multicolumn{3}{c|}{Fully supervised baseline} & $0.457\pm0.108$ & $0.559\pm 0.125 $ & $0.645 \pm0.101$ \\

 & \multicolumn{3}{c|}{SSDL baseline (no OOD data)} & $\mathbf{0.704 \pm 0.096}$ & $\mathbf{0.781\pm 0.065}$ & $\mathbf{0.831 \pm0.0626}$\\
 
 
 \cline{2-7}
 
 & \multirow{2}{*}{HH} & \multirow{2}{*}{OH} & 0 & $0.713\pm0.062$ & $0.802\pm0.064$ & $0.855\pm0.059$\\
 & & & 100 & $0.642 \pm 0.111$ & $0.746 \pm0.094$ & $0.798 \pm0.07$\\
 
 
 \cline{2-7}
 & \multirow{2}{*}{Sim} & \multirow{2}{*}{SVHN} & 50 & $0.637 \pm0.098$ & $0.745 \pm0.081$ & $0.801 \pm0.0699$\\
 
 & & & 100 & $0.482 \pm0.113$ & $0.719 \pm0.058$ & $0.765 \pm0.072$\\
 
  \cline{2-7}
 
  & \multirow{6}{*}{Dif}& \multirow{2}{*}{TI} & 50 & $0.642 \pm0.094$ & $0.739 \pm 0.074$ & $0.809 \pm0.066$\\
  
  & & & 100 & $0.637 \pm0.097$ & $0.732\pm 0.074$ & $0.804 \pm0.071$\\
  
  
 
 \cline{3-7}
 
  & & \multirow{2}{*}{G} & 50 & $0.606 \pm0.0989$ & $0.713 \pm0.087$ & $0.786\pm 0.065$\\
  
  & & & 100 & $0.442 \pm0.099$ & $0.461 \pm0.073$ & $0.542\pm 0.062$\\
  
 
  
   \cline{3-7}
 
  & & \multirow{2}{*}{SAP} & 50 & $0.631 \pm0.102$ & $0.735 \pm0.082$ & $0.813 \pm0.057$\\
  
  & & & 100 & $0.48\pm0.0951$ & $0.524 \pm0.09$ & $0.563 \pm0.095$\\
 
\midrule

\multirow{12}{*}{\rotatebox[origin=c]{90}{\textbf{CIFAR-10}}} & \multicolumn{3}{c|}{Fully supervised baseline} & $0.380\pm0.024$ & $0.445\pm0.042$ & $0.449\pm0.022$\\

 &  \multicolumn{3}{c|}{SSDL baseline (no OOD data)} & $\mathbf{0.453\pm0.046}$ & $0.474\pm0.019$ & $0.501\pm0.033$\\
 
 
 \cline{2-7}


& \multirow{2}{*}{HH} & \multirow{2}{*}{OH} & 50 & $0.444\pm0.040$ & $0.472\pm0.039$ & $0.525\pm0.050$\\ 
 & & & 100 & $0.443\pm0.023$ & $0.472\pm0.047$ & $0.499\pm0.054$ \\
 \cline{2-7}
 & \multirow{2}{*}{Sim} & \multirow{2}{*}{TI} & 50 & $0.435\pm0.054$ & $0.473\pm0.039$ & $\mathbf{0.543\pm0.040}$\\ 
 & & & 100 & $0.417\pm0.020$ & $\mathbf{0.480\pm0.039}$ & $0.498\pm0.042$ \\
 
 \cline{2-7}
 
  & \multirow{6}{*}{Dif} & \multirow{2}{*}{SVHN} & 50 & $0.419\pm0.027$ & $0.464\pm0.044$ & $0.469\pm0.056$\\ 
 & & & 100 & $0.385\pm0.034$ & $0.418\pm0.035$ & $0.440\pm0.046$ \\
 
 \cline{3-7}
 
  & & \multirow{2}{*}{G} & 50 & $0.409\pm0.047$ & $0.454\pm0.048$ & $0.491\pm0.032$\\ 
 & & & 100 & $0.297\pm0.029$ & $0.306\pm0.034$ & $0.302\pm0.038$ \\
 
 \cline{3-7}
 
  & & \multirow{2}{*}{SAP}& 50 & $0.438\pm0.029$ & $0.455\pm0.037$ & $0.485\pm0.034$\\ 
 & & & 100 & $0.236\pm0.031$ & $0.246\pm0.032$ & $0.232\pm0.022$ \\
  
  \midrule

\multirow{12}{*}{\rotatebox[origin=c]{90}{\textbf{FashionMNIST}}} & \multicolumn{3}{c|}{Fully supervised baseline} & $0.571\pm0.073$ & $0.704\pm0.066$ & $0.720\pm0.093$\\

 & \multicolumn{3}{c|}{SSDL baseline (no OOD data)} & $\mathbf{0.715\pm0.049}$ & $\mathbf{0.760\pm0.044}$ & $0.756\pm0.069$\\
 
 
 \cline{2-7}



& \multirow{2}{*}{HH} & \multirow{2}{*}{OH} & 50 & $0.714\pm0.049$ & $0.721\pm0.104$ & $0.765\pm0.053$\\ 
 & & & 100 & $0.660\pm0.061$ & $0.711\pm0.090$ & $0.747\pm0.061$ \\
 \cline{2-7}
 & \multirow{2}{*}{Sim} & \multirow{2}{*}{FP} & 50 & $0.707\pm0.039$ & $0.724\pm0.030$ & $0.778\pm0.078$\\ 
 & & & 100 & $0.546\pm0.101$ & $0.542\pm0.099$ & $0.540\pm0.105$ \\
 
 \cline{2-7}
 
  & \multirow{6}{*}{Dif}& \multirow{2}{*}{TI} & 50 & $0.690\pm0.065$ & $0.745\pm0.093$ & $0.792\pm0.058$\\ 
 & & & 100 & $0.690\pm0.073$ & $0.728\pm0.066$ & $\mathbf{0.794\pm0.056}$ \\
  
  \cline{3-7}
 
  & & \multirow{2}{*}{G} & 50 & $0.644\pm0.061$ & $0.689\pm0.075$ & $0.755\pm0.055$\\ 
 & & & 100 & $0.352\pm0.025$ & $0.366\pm0.065$ & $0.361\pm0.057$ \\
  
  \cline{3-7}
 
  & & \multirow{2}{*}{SAP} & 50 & $0.671\pm0.072$ & $0.708\pm0.095$ & $0.729\pm0.088$\\ 
 & & & 100 & $0.276\pm0.069$ & $0.297\pm0.046$ & $0.283\pm0.059$ \\
 
 \midrule

\multirow{12}{*}{\rotatebox[origin=c]{90}{\textbf{SVHN}}} & \multicolumn{3}{c|}{Fully supervised baseline} & $0.246\pm0.034$ & $0.253\pm0.021$ & $0.249\pm0.013$\\

 & \multicolumn{3}{c|}{SSDL baseline (no OOD data)} & $0.293\pm0.028$ & $0.332\pm0.050$ & $0.371\pm0.060$\\
 
 
 \cline{2-7}



& \multirow{2}{*}{HH} & \multirow{2}{*}{OH} & 50 & $0.307\pm0.048$ & $0.330\pm0.048$ & $0.380\pm0.048$\\ 
 & & & 100 & $0.307\pm0.053$ & $0.301\pm0.040$ & $0.398\pm0.055$ \\
 \cline{2-7}
 & \multirow{2}{*}{Sim} & \multirow{2}{*}{MNIST} & 50 & $0.296\pm0.040$ & $0.305\pm0.042$ & $0.293\pm0.043$\\ 
 & & & 100 & $0.287\pm0.040$ & $0.303\pm0.041$ & $0.274\pm0.028$ \\
 
 \cline{2-7}
 
  & \multirow{6}{*}{Dif} & \multirow{2}{*}{TI} & 50 & $\mathbf{0.339\pm0.047}$ & $0.361\pm0.048$ & $\mathbf{0.411\pm0.060}$\\ 
 & & & 100 & $0.323\pm0.056$ & $\mathbf{0.414\pm0.053}$ & $0.384\pm0.074$ \\
  
  \cline{3-7}
 
  & & \multirow{2}{*}{G} & 50 & $0.302\pm0.039$ & $0.360\pm0.040$ & $0.373\pm0.063$\\ 
 & & & 100 & $0.303\pm0.044$ & $0.284\pm0.050$ & $0.249\pm0.058$ \\
  
  \cline{3-7}
 
  & & \multirow{2}{*}{SAP} & 50 & $0.309\pm0.043$ & $0.332\pm0.033$ & $0.373\pm0.050$\\ 
 & & & 100 & $0.290\pm0.061$ & $0.294\pm0.070$ & $0.319\pm0.057$ \\


 \bottomrule
 
\end{tabular}

\end{small}
\end{center}
\end{table}
